RPMixer: Shaking Up Time Series Forecasting with Random Projections for Large Spatial-Temporal Data

Spatial-temporal forecasting systems play a crucial role in addressing numerous real-world challenges. In this paper, we investigate the potential of addressing spatial-temporal forecasting problems using general time series forecasting models, i.e., models that do not leverage the spatial relationships among the nodes. We propose a all-Multi-Layer Perceptron (all-MLP) time series forecasting architecture called RPMixer. The all-MLP architecture was chosen due to its recent success in time series forecasting benchmarks. Furthermore, our method capitalizes on the ensemble-like behavior of deep neural networks, where each individual block within the network behaves like a base learner in an ensemble model, particularly when identity mapping residual connections are incorporated. By integrating random projection layers into our model, we increase the diversity among the blocks' outputs, thereby improving the overall performance of the network. Extensive experiments conducted on the largest spatial-temporal forecasting benchmark datasets demonstrate that the proposed method outperforms alternative methods, including both spatial-temporal graph models and general forecasting models.

==> archive/insert/fig_benchmark_step.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_benchmark_step_0.pdf}
}
\caption{
The benchmark result measured using per-step MAE, RMSE, and MAPE.
Aside from the proposed method, we included only the five most effective methods from the Table~\ref{tab:largest_benchmark} to reduce clutter. 
The proposed method generally outperforms the alternatives more in later time steps compared to earlier ones.
}
\label{fig:benchmark_step}
\end{figure}

==> archive/insert/fig_param_layer_step_test.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_param_layer_step_test_0.pdf}
}
\caption{
The parameter sensitivity analysis for the \textit{number of block} parameter measured using per-step MAE, RMSE, and MAPE.
These results are derived from the test data. 
It was observed that this parameter has a more pronounced effect on later time steps compared to earlier ones.
}
\label{fig:param_layer_step_test}
\end{figure}

==> archive/insert/fig_param_layer_step_valid.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_param_layer_step_valid_0.pdf}
}
\caption{
The parameter sensitivity analysis for the \textit{number of block} parameter measured using per-step MAE, RMSE, and MAPE.
These results are derived from the validation data. 
It was observed that this parameter has a more pronounced effect on later time steps compared to earlier ones.
}
\label{fig:param_layer_step_valid}
\end{figure}

==> archive/insert/fig_param_neuron_step_test.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_param_neuron_step_test_0.pdf}
}
\caption{
The parameter sensitivity analysis for the \textit{number of neuron} parameter measured using per-step MAE, RMSE, and MAPE.
These results are derived from the test data. 
It was observed that this parameter has a more pronounced effect on later time steps compared to earlier ones.
}
\label{fig:param_neuron_step_test}
\end{figure}

==> archive/insert/fig_param_neuron_step_valid.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_param_neuron_step_valid_0.pdf}
}
\caption{
The parameter sensitivity analysis for the \textit{number of neuron} parameter measured using per-step MAE, RMSE, and MAPE.
These results are derived from the validation data. 
It was observed that this parameter has a more pronounced effect on later time steps compared to earlier ones.
}
\label{fig:param_neuron_step_valid}
\end{figure}

==> archive/insert/fig_unroll.tex <==
\begin{figure}[htp]
\centerline{
\includegraphics[width=0.85\linewidth]{insert/figure/fig_unroll_1.pdf}
}
\caption{
An illustrative example of an unraveled computational graph for the example network shown in Figure~\ref{fig:toy}, demonstrating the process of computing the final prediction.
}
\label{fig:unroll}
\end{figure}
